ELDEN: Exploration via Local Dependencies

Tasks with large state space and sparse rewards present a longstanding challenge to reinforcement learning. In these tasks, an agent needs to explore the state space efficiently until it finds a reward. To deal with this problem, the community has proposed to augment the reward function with intrinsic reward, a bonus signal that encourages the agent to visit interesting states. In this work, we propose a new way of defining interesting states for environments with factored state spaces and complex chained dependencies, where an agent's actions may change the value of one entity that, in order, may affect the value of another entity. Our insight is that, in these environments, interesting states for exploration are states where the agent is uncertain whether (as opposed to how) entities such as the agent or objects have some influence on each other. We present ELDEN, Exploration via Local DepENdencies, a novel intrinsic reward that encourages the discovery of new interactions between entities. ELDEN utilizes a novel scheme -- the partial derivative of the learned dynamics to model the local dependencies between entities accurately and computationally efficiently. The uncertainty of the predicted dependencies is then used as an intrinsic reward to encourage exploration toward new interactions. We evaluate the performance of ELDEN on four different domains with complex dependencies, ranging from 2D grid worlds to 3D robotic tasks. In all domains, ELDEN correctly identifies local dependencies and learns successful policies, significantly outperforming previous state-of-the-art exploration methods.

==> backup/backup.tex <==
% Original intro:
Learning an accurate dynamic model is a key goal for model-based reinforcement learning (MBRL). Previous work by \citet{wang2021causal} showed that identifying causal relationships between state variables improves the quality of the learned dynamics model as well as its generalizability to out-of-distribution states, compared to not using causal dependencies. 
However, \citet{wang2021causal} only considers global causal relations between variables, which can often be relatively dense and hard to disentangle. 
In this work, we investigate how local (i.e., state-dependent) causal relationships in a dynamics system can be learned and exploited for accurate and generalizable models. Our key motivation is that causal dependencies between state variables are often sparse in a dynamics system. Consider the case where a robot is trying to open a door: in most of the transitions, the robot's action has no influence the door, and the door only depends on the robot when they are in contact. Our goal is to uncover such sparse state-dependent causal relationships to learn accurate dynamics model. 

In contrast to \cite{wang2021causal} which relies on conditional independence tests that only infers global (state-independent) causal relationships, we propose to use gradient penalties to learn local relationships. Specifically, we want to learn a causal dynamics model which predict the next state $s_{t+1}$ based on the current state $s_t$ and action $a_t$, under the soft constraint that non-zero gradient entries of $s_{t+1}$ with respect to $s_t$ should be as few as possible. With this constraint, our model is encouraged to remove unnecessary dependencies between state variables at the given state, and thereby learn a local causal dynamics model. To extract local causal graph from the learned dynamic model, we propose to perturb the input states with small noise, and use the average gradient magnitude as a target score, which effectively give us a smooth gradient estimation.

Our preliminary results show that using smooth gradient causality extractor on dynamic models trained with the gradient penalty objective allows us to relatively accurately identify local connectivity between state variables. We plan to provide more comparison of our method with previous methods, as well as demonstration of how the local causality can be used to improve down-stream tasks, in the final project report.

%From method section
Our key idea is to utilize gradient penalty to encourage sparse connectivity from current state and action to next state, thereby enforcing a \textbf{locally sparse} causal dynamic model. Specifically, 
like most MBRL algorithsm, we first collect a dataset of the environment transitions using some pre-defined data collection method (we used HiPPO \cite{li2019sub} in our work). Next, we train dynamic model by minimizing the prediction error, with an additional gradient penalty term that penalize the manitude of the gradient from input to the output, i.e. $L_{\theta} = L_{\text{pred}} + L_{\text{grad}}$. Our network architecture follows \citet{wang2021causal}. We will provide more detail of our approach in the final project report. 

==> backup/deleted.tex <==

% \begin{algorithm}[tb]
%  \caption{Training of off-policy \methodname{}}
%  \label{algorithm}
%  \begin{algorithmic}[1]\small
%   \State Initialize the dynamics ensemble $\{f\}^N$, policy $\pi_\theta$, and replay buffer $D$.
%   \For {number of training iterations}
%     \State Sample action $a \sim \pi_\theta(x)$
%     \State Collect environment step $s\text{'}, r_{\text{task}} \sim \text{env}(s, a)$
%     \State Add $s, a, r_{\text{task}}, s\text{'}$ into the replay buffer $D$
%     \State Sample a mini-batch $B = \{s, a, r_{\text{task}}, s\text{'}\}^K$ from $D$
%     \State Train the dynamics ensemble $\{f\}^N$ with the mini-batch (sec.~\ref{sec:dl})
%     \State Compute the intrinsic reward as the variance of the locality dependencies graph:
%     \State $\ \ \ \ \ \ \ LC^{k,n} = f^n.compute\_LC(s^k, a^k)$ (sec.~\ref{sec:dl})
%         \State $\ \ \ \ \ \ \ r^k_{\text{intrinsic}} = \text{variance}(\{LC^{k,n}\})$
%         \State $\ \ \ \ \ \ \  r^k = r^k_{\text{task}} + \lambda \cdot r^k_{\text{intrinsic}}$
%     \State Update the policy $\pi_\theta$ with the mini-batch $B = \{s, a, r, s\text{'}\}^K$
%  \EndFor
%  \end{algorithmic} 
%  \end{algorithm}

==> backup/intro_backup0516.tex <==
\section{Introduction}


Reinforcement learning (RL) has achieved remarkable success in recent years in tasks where a well-shaped dense reward function is naturally available, such as playing video games~\citep{mnih2015human, wurman2022outracing} and controlling robots~\citep{haarnoja2018learning, andrychowicz2020learning}\roberto{add more citations}. However, for sparse reward tasks where the agent receives no signal for most of the transitions collected, learning good policies remains difficult. In these tasks, the challenge becomes exploring the state space efficiently without any reward signal, the so-called hard-exploration problem~\citep{yang2021exploration}.

% A critical reason for such difficulty is the challenge of sufficiently exploring the state space even when reward signals are lacking, also known as the hard-exploration problem~\citep{yang2021exploration}. 

RL researchers have tackled the hard-exploration problem by introducing an intrinsic reward: providing the agent an additional reward signal for visiting ``interesting states''. Prior works explored alternative ways to define whether a state is interesting or not~\citep{bellemare2016unifying, tang2017exploration, stadie2015incentivizing, pathak2017curiosity, schmidhuber1991possibility, burda2018exploration, seitzer2021causal} leading to two main paradigms: curiosity and empowerment. In curiosity-driven exploration, a state is considered ``interesting'' if the prediction error or uncertainty of the state~\citep{pathak2019self, bellemare2016unifying} or some state features~\citep{burda2018exploration, pathak2017curiosity} is high. However, learning accurate models of the dynamics requires significantly covering the state-action space with experiences, and it is affected by the level of stochasticity of the environment. On the other hand, in empowerment-based exploration, ``interesting states'' are those where the agent obtains maximal control of the environment through actions~\citep{seitzer2021causal, zhao2021mutual}, measured as the mutual information (MI) between actions and states. \roberto{I'd talk here about other limitations of empowerment-based exploration and leave this one to the next paragraph, where the special type of environment/task is explained and then it can be understood how these methods fail. afaik, EBE is hard to compute and has been demonstrated only for simple tasks. any more fundamental limitations?}
Empowerment-based methods have been demonstrated on simple tasks, where computing the MI is feasible.
Moreover, empowerment does not encourage exploring the entire state space but rather finding a state where the agent can choose between multiple alternative futures.
% Besides the difficulties of computing MI, empowerment-based exploration only considers direct dependencies between actions and states and ignores state-to-state dependencies.

While effective in some scenarios, these methods struggle in environments with rich and complex interactions between elements of the environment like objects (see details in Sec.~\ref{}).
Consider the example where a robot needs to cook a meatball on the stove (Fig.~\ref{fig:pan}). Both families of prior methods would keep oscillating the pan to make the meatball roll: for curiosity-driven methods, this behavior gives high rewards for hard-to-predict meatball movement; for empowerment-driven methods, manipulating the pan and the meatball gives a high controllability reward. By contrast, after a few trials, humans figure out that they can use the pan to move the meatball. Then, instead of spending time learning the complex meatball movement or different styles to manipulate the pan, humans would move on to explore interactions with different objects, e.g., putting the pan on the stove and switching on the stove. \roberto{the example is good but feels a bit too high level. for example, what is the real task? if the task would be to control the position of the meatball, what the sota methods do would be good. but because the task is another (long horizon? involving multiple changes of interaction modes?) that exploration is inefficient compared to ours. The task nature needs to be clear to understand the example and the underlying idea}

Our key insight is humans tend to use novel interaction modes between environment entities as inductive bias to improve exploration, especially in environments with rich interaction possibilities, as illustrated in the meatball example.\roberto{dangerous. I would not say what humans do, that is cognitive science. I would rather say something like "intelligent (or efficient) exploration emerges when an agent uses interaction modes as inductive bias to improve exploration, ..."}
Inspired by how humans explore, we present \textbf{E}xploration via \textbf{L}ocal \textbf{D}ep\textbf{EN}dencies (\methodname{}), a novel intrinsic reward mechanism that models the local dependencies between entities in the scene and uses the uncertainty about the dependencies to encourage exploration. 
By relaxing the curiosity signal from dynamics prediction to dependencies prediction, \methodname{} implicitly encourages the model to pay closer attention to states where novel interaction happens, and lesser attention to states where only the state values are novel.
% Dependencies are easier to predict accurately than dynamics, which often requires low-level, fine-grained predictions...
Specifically, \methodname{} trains an ensemble of dynamics models. In each model, the local dependencies between objects are modeled by the partial derivatives of state predictions w.r.t. the current state and action. Then, the local dependency uncertainty is measured as the variance across all dynamic models.

We evaluate \methodname{} on discrete and continuous domains with complex interactions that require long-horizon reasoning. Our results show that using a gradient dependencies extractor on dynamic models training allows us to accurately identify local connectivities between environment entities. Furthermore, the intrinsic reward derived from the identified local connectivities allows \methodname{} to outperform state-of-the-art exploration methods during the training of RL agents, both in sample efficiency and convergence performance.






% While building intrinsic rewards based on state features has achieved remarkable success, they mostly focus on low-level dynamics, i.e., fine-grain prediction of object movements. Humans, by contrast, are often interested in high-level abstract dynamics, i.e., whether the action can influence an object or whether there are influences among objects. 
% Consider the example shown in Fig.~\ref{fig:pan}, where an agent needs to heat a piece of bread by turning on the stove, putting bread inside the pan, and then putting the pan onto the stove. A human can relatively easily figure out that the interesting states would be when the bread is put inside the pan on a stove that is turned on since this is the only state in which the stove is interacting with the bread. However, an intrinsic reward based on an inverse dynamics model such as in \citet{pathak2017curiosity} would not be interested in getting the bread heated since the agent's action has no effect on the state of the bread during the heating process. On the other hand, using a forward dynamics model such as \citet{stadie2015incentivizing} may suffer from irrelevant noise in the observation, known as the "noisy TV'' problem, where variations such as lighting conditions may dominate the intrinsic reward signal.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{images/comparison_ph.png}
    \caption{\small We are interested in tasks where there are complex interactions between objects, such as the one shown in this figure. In this task, a robot needs to cook the meatball in the pan on the stove.  
    Curiosity-based methods may focus on states with challenging predictions, such as the rolling motion of the meatball.
    On the other hand, empowerment-based methods would not be interested in cooking the meatball as the agent will have no effect on the pan and the meatball when they are placed on the stove.  
    \methodname{} avoids both issues by explicitly modeling the interactions between environment entities and using it to encourage exploration.}
    \label{fig:pan}
\end{figure}
